Imperfect Is Perfect: Learned Column Prefilling for Branch-Price-and-Cut

Column generation folklore warns that initial columns hurt: a warm start may bias the dual and slow the root of branch-price-and-cut. We show the opposite once the columns are imperfect in the right way. Preloading the support of the optimal root LP, the best columns one could know in advance, fails to finish on half of our hardest instances; a pool of ordinary routes that need not belong to any optimal solution, held outside the master and priced at the current smoothed dual, speeds the root up. Because the columns need not be optimal, producing them becomes a learning task: a neural edge scorer guides a constructive generator that builds the pool in seconds. A second network predicts the initial center of Wentges smoothing from the instance file, and with it the direction of the smoothed pricing queries; the solver's own updates run unchanged. With prefill and center in place, exact pricing dominates root pricing time, so we rebuild bucket-graph labeling around its dominance test for the GPU and certify on the CPU. Inside RouteOpt, the state-of-the-art exact solver for capacitated vehicle routing, the pipeline reaches the same certified root bound in 13.2% of vanilla RouteOpt's root pricing time over 95 instances with 300 to 1000 customers, prefill alone in 26.1%, and 17.5 times faster in the best case. In an exact branch-price-and-cut solver for unrelated parallel machine scheduling, prefill with smoothing and the learned center certifies all 25 benchmark instances, 12 times faster than the solver's own column generation, which certifies 20 of them.

==> sections/appD_tables.tex <==
\newcommand{\appDTabOneRows}{%
X-n327-k20 & 326 & 20 & 112.6 & 31.5 & 48.8 & 34.9 & 43.2 & 12.6 & 77.9 \\
X-n367-k17 & 366 & 17 & 453.2 & 184.3 & 201.3 & 167.6 & 171.9 & 108.2 & $\ge$\,955.4 \\
X-n449-k29 & 448 & 29 & 611.3 & 200.2 & 253.0 & 200.7 & 230.6 & 85.2 & 317.4 \\
X-n513-k21 & 512 & 21 & 955.8 & 325.2 & 368.3 & 461.4 & 412.4 & 308.2 & $\ge$\,1672 \\
X-n561-k42 & 560 & 42 & 438.7 & 74.5 & 100.1 & 80.5 & 107.1 & 61.7 & 347.1 \\
X-n641-k35 & 640 & 35 & 1251 & 524.5 & 661.9 & 579.5 & 697.2 & 187.2 & 879.0 \\
X-n783-k48 & 782 & 48 & 4076 & 1222 & 1144 & 1210 & 1101 & 634.8 & $\ge$\,6478 \\
X-n801-k40 & 800 & 40 & 1024 & 309.7 & 498.7 & 312.4 & 518.7 & 156.1 & $\ge$\,1841 \\
X-n979-k58 & 978 & 58 & 13017 & 4490 & 4955 & 4931 & 4670 & 1954 & 13695 \\
X-n1001-k43 & 1000 & 43 & 7287 & 1825 & 2171 & 1498 & 2051 & 3461 & $\ge$\,11399 \\}
\newcommand{\appDOnePnGM}{0.305}
\newcommand{\appDOnePnN}{10}
\newcommand{\appDOnePnWins}{10}
\newcommand{\appDOnePnCensoredN}{0}
\newcommand{\appDOnePnCI}{[0.263, 0.355]}
\newcommand{\appDOnePhGM}{0.377}
\newcommand{\appDOnePhN}{10}
\newcommand{\appDOnePhWins}{10}
\newcommand{\appDOnePhCensoredN}{0}
\newcommand{\appDOnePhCI}{[0.323, 0.439]}
\newcommand{\appDOnePdumpGM}{0.319}
\newcommand{\appDOnePdumpN}{10}
\newcommand{\appDOnePdumpWins}{10}
\newcommand{\appDOnePdumpCensoredN}{0}
\newcommand{\appDOnePdumpCI}{[0.266, 0.382]}
\newcommand{\appDOnePhdumpGM}{0.367}
\newcommand{\appDOnePhdumpN}{10}
\newcommand{\appDOnePhdumpWins}{10}
\newcommand{\appDOnePhdumpCensoredN}{0}
\newcommand{\appDOnePhdumpCI}{[0.315, 0.429]}
\newcommand{\appDOnePconvGM}{0.183}
\newcommand{\appDOnePconvN}{10}
\newcommand{\appDOnePconvWins}{10}
\newcommand{\appDOnePconvCensoredN}{0}
\newcommand{\appDOnePconvCI}{[0.141, 0.238]}
\newcommand{\appDOnePsuppGM}{0.732}
\newcommand{\appDOnePsuppN}{5}
\newcommand{\appDOnePsuppWins}{4}
\newcommand{\appDOnePsuppCensoredN}{5}
\newcommand{\appDOnePsuppCI}{[0.574, 0.934]}
\newcommand{\appDTabOneGMRow}{\textbf{GM of ratio to vanilla} & & & 1 & 0.305 & 0.377 & 0.319 & 0.367 & 0.183 & 0.732\,(5 censored) \\}
\newcommand{\appDTabOneWinsRow}{wins ($<$ vanilla) & & & & 10/10 & 10/10 & 10/10 & 10/10 & 10/10 & 4/10 \\}
\newcommand{\appDOnePnOverPhGM}{0.811}
\newcommand{\appDOnePnOverPhN}{10}
\newcommand{\appDOnePhBeatsPnN}{1}
\newcommand{\appDOnePnOverPhCI}{[0.737, 0.892]}
\newcommand{\appDOnePnOverPdumpGM}{0.958}
\newcommand{\appDOnePnOverPdumpN}{10}
\newcommand{\appDOnePdumpBeatsPnN}{3}
\newcommand{\appDOnePnOverPdumpCI}{[0.881, 1.041]}
\newcommand{\appDOnePnOverPhdumpGM}{0.832}
\newcommand{\appDOnePnOverPhdumpN}{10}
\newcommand{\appDOnePhdumpBeatsPnN}{2}
\newcommand{\appDOnePnOverPhdumpCI}{[0.742, 0.932]}
\newcommand{\appDOnePnOverPconvGM}{1.666}
\newcommand{\appDOnePnOverPconvN}{10}
\newcommand{\appDOnePconvBeatsPnN}{9}
\newcommand{\appDOnePnOverPconvCI}{[1.240, 2.239]}
\newcommand{\appDOnePnOverPsuppGM}{0.404}
\newcommand{\appDOnePnOverPsuppN}{5}
\newcommand{\appDOnePsuppBeatsPnN}{0}
\newcommand{\appDOnePnOverPsuppCI}{[0.264, 0.617]}
\newcommand{\appDOnePhOverPnGM}{1.233}
\newcommand{\appDOnePhOverPnN}{10}
\newcommand{\appDOnePnBeatsPhN}{9}
\newcommand{\appDOnePhOverPnCI}{[1.121, 1.356]}
\newcommand{\appDOnePhOverPdumpGM}{1.181}
\newcommand{\appDOnePhOverPdumpN}{10}
\newcommand{\appDOnePdumpBeatsPhN}{8}
\newcommand{\appDOnePhOverPdumpCI}{[1.045, 1.334]}
\newcommand{\appDOnePhOverPhdumpGM}{1.026}
\newcommand{\appDOnePhOverPhdumpN}{10}
\newcommand{\appDOnePhdumpBeatsPhN}{6}
\newcommand{\appDOnePhOverPhdumpCI}{[0.974, 1.080]}
\newcommand{\appDOnePhOverPconvGM}{2.054}
\newcommand{\appDOnePhOverPconvN}{10}
\newcommand{\appDOnePconvBeatsPhN}{9}
\newcommand{\appDOnePhOverPconvCI}{[1.482, 2.847]}
\newcommand{\appDOnePhOverPsuppGM}{0.523}
\newcommand{\appDOnePhOverPsuppN}{5}
\newcommand{\appDOnePsuppBeatsPhN}{0}
\newcommand{\appDOnePhOverPsuppCI}{[0.339, 0.808]}
\newcommand{\appDOnePdumpOverPnGM}{1.044}
\newcommand{\appDOnePdumpOverPnN}{10}
\newcommand{\appDOnePnBeatsPdumpN}{7}
\newcommand{\appDOnePdumpOverPnCI}{[0.960, 1.135]}
\newcommand{\appDOnePdumpOverPhGM}{0.847}
\newcommand{\appDOnePdumpOverPhN}{10}
\newcommand{\appDOnePhBeatsPdumpN}{2}
\newcommand{\appDOnePdumpOverPhCI}{[0.750, 0.957]}
\newcommand{\appDOnePdumpOverPhdumpGM}{0.869}
\newcommand{\appDOnePdumpOverPhdumpN}{10}
\newcommand{\appDOnePhdumpBeatsPdumpN}{3}
\newcommand{\appDOnePdumpOverPhdumpCI}{[0.773, 0.976]}
\newcommand{\appDOnePdumpOverPconvGM}{1.740}
\newcommand{\appDOnePdumpOverPconvN}{10}
\newcommand{\appDOnePconvBeatsPdumpN}{9}
\newcommand{\appDOnePdumpOverPconvCI}{[1.255, 2.412]}
\newcommand{\appDOnePdumpOverPsuppGM}{0.435}
\newcommand{\appDOnePdumpOverPsuppN}{5}
\newcommand{\appDOnePsuppBeatsPdumpN}{0}
\newcommand{\appDOnePdumpOverPsuppCI}{[0.288, 0.657]}
\newcommand{\appDOnePhdumpOverPnGM}{1.202}
\newcommand{\appDOnePhdumpOverPnN}{10}
\newcommand{\appDOnePnBeatsPhdumpN}{8}
\newcommand{\appDOnePhdumpOverPnCI}{[1.073, 1.347]}
\newcommand{\appDOnePhdumpOverPhGM}{0.975}
\newcommand{\appDOnePhdumpOverPhN}{10}
\newcommand{\appDOnePhBeatsPhdumpN}{4}
\newcommand{\appDOnePhdumpOverPhCI}{[0.926, 1.027]}
\newcommand{\appDOnePhdumpOverPdumpGM}{1.151}
\newcommand{\appDOnePhdumpOverPdumpN}{10}
\newcommand{\appDOnePdumpBeatsPhdumpN}{7}
\newcommand{\appDOnePhdumpOverPdumpCI}{[1.025, 1.293]}
\newcommand{\appDOnePhdumpOverPconvGM}{2.003}
\newcommand{\appDOnePhdumpOverPconvN}{10}
\newcommand{\appDOnePconvBeatsPhdumpN}{9}
\newcommand{\appDOnePhdumpOverPconvCI}{[1.450, 2.766]}
\newcommand{\appDOnePhdumpOverPsuppGM}{0.507}
\newcommand{\appDOnePhdumpOverPsuppN}{5}
\newcommand{\appDOnePsuppBeatsPhdumpN}{0}
\newcommand{\appDOnePhdumpOverPsuppCI}{[0.337, 0.765]}
\newcommand{\appDOnePconvOverPnGM}{0.600}
\newcommand{\appDOnePconvOverPnN}{10}
\newcommand{\appDOnePnBeatsPconvN}{1}
\newcommand{\appDOnePconvOverPnCI}{[0.447, 0.807]}
\newcommand{\appDOnePconvOverPhGM}{0.487}
\newcommand{\appDOnePconvOverPhN}{10}
\newcommand{\appDOnePhBeatsPconvN}{1}
\newcommand{\appDOnePconvOverPhCI}{[0.351, 0.675]}
\newcommand{\appDOnePconvOverPdumpGM}{0.575}
\newcommand{\appDOnePconvOverPdumpN}{10}
\newcommand{\appDOnePdumpBeatsPconvN}{1}
\newcommand{\appDOnePconvOverPdumpCI}{[0.415, 0.797]}
\newcommand{\appDOnePconvOverPhdumpGM}{0.499}
\newcommand{\appDOnePconvOverPhdumpN}{10}
\newcommand{\appDOnePhdumpBeatsPconvN}{1}
\newcommand{\appDOnePconvOverPhdumpCI}{[0.362, 0.689]}
\newcommand{\appDOnePconvOverPsuppGM}{0.188}
\newcommand{\appDOnePconvOverPsuppN}{5}
\newcommand{\appDOnePsuppBeatsPconvN}{0}
\newcommand{\appDOnePconvOverPsuppCI}{[0.149, 0.238]}
\newcommand{\appDOnePsuppOverPnGM}{2.478}
\newcommand{\appDOnePsuppOverPnN}{5}
\newcommand{\appDOnePnBeatsPsuppN}{5}
\newcommand{\appDOnePsuppOverPnCI}{[1.620, 3.790]}
\newcommand{\appDOnePsuppOverPhGM}{1.911}
\newcommand{\appDOnePsuppOverPhN}{5}
\newcommand{\appDOnePhBeatsPsuppN}{5}
\newcommand{\appDOnePsuppOverPhCI}{[1.237, 2.952]}
\newcommand{\appDOnePsuppOverPdumpGM}{2.298}
\newcommand{\appDOnePsuppOverPdumpN}{5}
\newcommand{\appDOnePdumpBeatsPsuppN}{5}
\newcommand{\appDOnePsuppOverPdumpCI}{[1.523, 3.467]}
\newcommand{\appDOnePsuppOverPhdumpGM}{1.971}
\newcommand{\appDOnePsuppOverPhdumpN}{5}
\newcommand{\appDOnePhdumpBeatsPsuppN}{5}
\newcommand{\appDOnePsuppOverPhdumpCI}{[1.307, 2.971]}
\newcommand{\appDOnePsuppOverPconvGM}{5.318}
\newcommand{\appDOnePsuppOverPconvN}{5}
\newcommand{\appDOnePconvBeatsPsuppN}{5}
\newcommand{\appDOnePsuppOverPconvCI}{[4.202, 6.730]}
\newcommand{\appDOneInstN}{10}
\newcommand{\appDOneDoneN}{10}
\newcommand{\appDTabTwoRows}{%
X-n327-k20 & 326 & 20 & 112.6 & 115.1 & 93.8 & 73.2 \\
X-n367-k17 & 366 & 17 & 453.2 & 343.2 & 312.8 & 368.9 \\
X-n449-k29 & 448 & 29 & 611.3 & 487.7 & 430.0 & 340.1 \\
X-n513-k21 & 512 & 21 & 955.8 & 817.8 & 686.2 & 542.7 \\
X-n561-k42 & 560 & 42 & 438.7 & 397.0 & 333.1 & 260.2 \\
X-n641-k35 & 640 & 35 & 1251 & 1119 & 856.5 & 774.3 \\
X-n783-k48 & 782 & 48 & 4076 & 3515 & 2988 & 2487 \\
X-n801-k40 & 800 & 40 & 1024 & 966.3 & 843.5 & 732.6 \\
X-n979-k58 & 978 & 58 & 13017 & 7623 & 7048 & 5667 \\
X-n1001-k43 & 1000 & 43 & 7287 & 6015 & 5421 & 4534 \\}
\newcommand{\appDTwoSGM}{0.837}
\newcommand{\appDTwoSN}{10}
\newcommand{\appDTwoSWins}{9}
\newcommand{\appDTwoSCensoredN}{0}
\newcommand{\appDTwoSCI}{[0.766, 0.914]}
\newcommand{\appDTwoCrandGM}{0.719}
\newcommand{\appDTwoCrandN}{10}
\newcommand{\appDTwoCrandWins}{10}
\newcommand{\appDTwoCrandCensoredN}{0}
\newcommand{\appDTwoCrandCI}{[0.670, 0.770]}
\newcommand{\appDTwoCnGM}{0.611}
\newcommand{\appDTwoCnN}{10}
\newcommand{\appDTwoCnWins}{10}
\newcommand{\appDTwoCnCensoredN}{0}
\newcommand{\appDTwoCnCI}{[0.556, 0.672]}
\newcommand{\appDTabTwoGMRow}{\textbf{GM of ratio to vanilla} & & & 1 & 0.837 & 0.719 & 0.611 \\}
\newcommand{\appDTabTwoWinsRow}{wins ($<$ vanilla) & & & & 9/10 & 10/10 & 10/10 \\}
\newcommand{\appDTwoSOverCrandGM}{1.164}
\newcommand{\appDTwoSOverCrandN}{10}
\newcommand{\appDTwoCrandBeatsSN}{10}
\newcommand{\appDTwoSOverCrandCI}{[1.126, 1.204]}
\newcommand{\appDTwoSOverCnGM}{1.369}
\newcommand{\appDTwoSOverCnN}{10}
\newcommand{\appDTwoCnBeatsSN}{9}
\newcommand{\appDTwoSOverCnCI}{[1.257, 1.492]}
\newcommand{\appDTwoCrandOverSGM}{0.859}
\newcommand{\appDTwoCrandOverSN}{10}
\newcommand{\appDTwoSBeatsCrandN}{0}
\newcommand{\appDTwoCrandOverSCI}{[0.831, 0.888]}
\newcommand{\appDTwoCrandOverCnGM}{1.176}
\newcommand{\appDTwoCrandOverCnN}{10}
\newcommand{\appDTwoCnBeatsCrandN}{9}
\newcommand{\appDTwoCrandOverCnCI}{[1.094, 1.264]}
\newcommand{\appDTwoCnOverSGM}{0.730}
\newcommand{\appDTwoCnOverSN}{10}
\newcommand{\appDTwoSBeatsCnN}{1}
\newcommand{\appDTwoCnOverSCI}{[0.670, 0.796]}
\newcommand{\appDTwoCnOverCrandGM}{0.850}
\newcommand{\appDTwoCnOverCrandN}{10}
\newcommand{\appDTwoCrandBeatsCnN}{1}
\newcommand{\appDTwoCnOverCrandCI}{[0.791, 0.914]}
\newcommand{\appDTwoInstN}{10}
\newcommand{\appDTwoDoneN}{10}
\newcommand{\appDPoolSizeRows}{%
X-n327-k20 & 164928 & 19 & 15075 & 10 & 9739 & 242 \\
X-n367-k17 & 128367 & 9 & 8055 & 10 & 8660 & 256 \\
X-n449-k29 & 166851 & 20 & 13711 & 10 & 6817 & 373 \\
X-n513-k21 & 163265 & 21 & 12912 & 10 & 7758 & 339 \\
X-n561-k42 & 199585 & 20 & 17717 & 10 & 9504 & 423 \\
X-n641-k35 & 200977 & 17 & 9745 & 10 & 7876 & 529 \\
X-n783-k48 & 228361 & 24 & 8727 & 10 & 7321 & 622 \\
X-n801-k40 & 159933 & 21 & 5780 & 10 & 9160 & 529 \\
X-n979-k58 & 66662 & 16 & 4145 & 10 & 8589 & 788 \\
X-n1001-k43 & 326470 & 24 & 2185 & 10 & 9895 & 738 \\}
\newcommand{\appDGenPnMin}{9}
\newcommand{\appDGenPnMax}{24}
\newcommand{\appDGenPhMin}{10}
\newcommand{\appDGenPhMax}{10}


==> sections/app_bpc.tex <==
\section{Branch-price-and-cut in detail}
\label{app:bpc}

This appendix defines the routing and scheduling masters, their pricing problems and the
associated bounds: the master problem obtained by Dantzig--Wolfe decomposition, the primal--dual
relations that make pricing a separation problem and give every dual point a bound, and the two
pricing problems on which the paper's components are evaluated. Throughout, $v=(u,\sigma)$ denotes the full dual vector of a master,
$u$ the block of multipliers on the covering rows and $\sigma$ the multiplier of the resource-count
row; where that row is absent, $\sigma$ is omitted.

\subsection{Dantzig--Wolfe decomposition and the master problem}
\label{app:bpc-dw}

Let the compact model have $K$ blocks coupled by linking constraints,
\begin{equation}
z_{\mathrm{IP}}=\min\Big\{\sum_{k=1}^{K} c_k^{\top}x_k:\ \sum_{k=1}^{K} A_k x_k = b,\ \
x_k\in X_k\ (k=1,\dots,K)\Big\},
\label{eq:app-compact}
\end{equation}
where $X_k=\{x\in\mathbb{Z}^{n_k}_{\ge 0}:\ D_k x\le d_k\}$ is bounded for every $k$.
Write $X_k=\{x_{k,r}:\ r\in R_k\}$ for the finite point set of block $k$. Every
$x_k\in\operatorname{conv}(X_k)$ is a convex combination $x_k=\sum_{r\in R_k}\lambda_{k,r}x_{k,r}$
with $\sum_{r\in R_k}\lambda_{k,r}=1$ and $\lambda_k\ge 0$ \citep{dantzig1960decomposition}.
Substituting into \eqref{eq:app-compact} gives the \emph{master LP}
\begin{equation}
z_{\mathrm{DW}}=\min_{\lambda\ge 0}\Big\{\sum_{k}\sum_{r\in R_k} c_{k,r}\lambda_{k,r}:\
\sum_{k}\sum_{r\in R_k} a_{k,r}\lambda_{k,r}=b,\ \
\sum_{r\in R_k}\lambda_{k,r}=1\ (k=1,\dots,K)\Big\},
\label{eq:app-master-dw}
\end{equation}
with $c_{k,r}=c_k^{\top}x_{k,r}$ and $a_{k,r}=A_kx_{k,r}$. Requiring in addition
$\sum_r\lambda_{k,r}x_{k,r}\in X_k$, which for the set-partitioning structures below is the
integrality of $\lambda$, gives the integer master, whose optimum is $z_{\mathrm{IP}}$.

\begin{proposition}[Dantzig--Wolfe bound]
\label{prop:app-dw}
Let $z_{\mathrm{LP}}$ be the value of \eqref{eq:app-compact} with each $X_k$ replaced by
$\{x\ge 0:\ D_kx\le d_k\}$, and let
$z_{\mathrm{L}}=\max_{\mu}\big[\mu^{\top}b+\sum_k\min\{(c_k-A_k^{\top}\mu)^{\top}x_k:\ x_k\in X_k\}\big]$
be the Lagrangian dual of the linking constraints. Then
$z_{\mathrm{LP}}\le z_{\mathrm{DW}}=z_{\mathrm{L}}\le z_{\mathrm{IP}}$, and
$z_{\mathrm{LP}}=z_{\mathrm{DW}}$ whenever every polyhedron $\{x\ge 0:\ D_kx\le d_k\}$ has integral
vertices.
\end{proposition}
\begin{proof}
Problem \eqref{eq:app-master-dw} minimizes the objective of \eqref{eq:app-compact} over
$\prod_k\operatorname{conv}(X_k)$, which is contained in $\prod_k\{x\ge 0:\ D_kx\le d_k\}$ and
equals it when the vertices are integral; this gives the first inequality and the equality case.
LP duality applied to \eqref{eq:app-master-dw}, with $\mu$ the multipliers of the linking rows and
the convexity rows priced out block by block, gives $z_{\mathrm{DW}}=z_{\mathrm{L}}$, and
$z_{\mathrm{L}}\le z_{\mathrm{IP}}$ is weak Lagrangian duality \citep{lubbecke2005selected}.
\end{proof}

\paragraph{Aggregation and the routing master.}
Aggregating $K$ identical blocks, as the vehicles of one fleet are, drops the block index, makes
a column the plan of one anonymous block, and turns the $K$ convexity rows into a single equation
counting the selected plans. For the CVRP with a free fleet, RouteOpt instead uses the valid
vehicle-count inequality $\sum_r\lambda_r\ge K_{\min}$, with $K_{\min}$ a lower bound on the
number of vehicles; adding this row to \eqref{eq:master} gives the following master and its dual,
\begin{equation}
\begin{aligned}
z_{\mathrm{DW}}\;=\;&\min_{\lambda\ge 0}\Big\{\sum_{r\in\mathcal R} c_r\lambda_r:\
\sum_{r\in\mathcal R} a_{ir}\lambda_r = 1\ (i\in C),\ \ \sum_{r\in\mathcal R}\lambda_r\ge K_{\min}\Big\}\\
\;=\;&\max_{u\in\mathbb R^{n},\ \sigma\ge 0}\Big\{\sum_{i\in C}u_i+K_{\min}\sigma:\
rc_r(v)=c_r-a_r^{\top}u-\sigma\ \ge\ 0,\ \ r\in\mathcal R\Big\},
\end{aligned}
\label{eq:app-cvrp-master}
\end{equation}
where $\mathcal R$ is the set of ng-feasible routes of Appendix~\ref{app:bpc-cvrp}, $c_r$ the
length of route $r$ and $a_{ir}$ its number of visits to customer $i$. Unrelated machines are not
copies of one another, and the scheduling master of Appendix~\ref{app:bpc-upms} keeps one row per
machine.

\subsection{Column generation: the primal--dual view}
\label{app:bpc-cg}

\paragraph{Restricted master and pricing.}
For a route set $T\subseteq\mathcal R$ containing all singleton routes, let $\mathrm{RMP}(T)$ be
\eqref{eq:app-cvrp-master} with $\mathcal R$ replaced by $T$, let $z_T$ be its value, $\lambda_T$
a basic optimal solution and $v_T=(u_T,\sigma_T)$ the associated basic optimal dual. Extending the
notation of \eqref{eq:dualpoly} to the vehicle row, let
\begin{equation}
D_T=\{(u,\sigma)\in\mathbb R^{n}\times\mathbb R_{\ge 0}:\ a_r^{\top}u+\sigma\le c_r,\ r\in T\},
\qquad
F_T=\arg\max_{(u,\sigma)\in D_T}\Big\{\sum_{i\in C}u_i+K_{\min}\sigma\Big\},
\label{eq:app-dualpoly}
\end{equation}
so that $v_T$ is a vertex of $F_T$ and $D_{\mathcal R}$ is the feasible set of the full dual. The
\emph{pricing problem} at a dual point $v$ is
\begin{equation}
m(v)\;=\;\min_{r\in\mathcal R}\ rc_r(v),\qquad rc_r(v)=c_r-a_r^{\top}u-\sigma ,
\label{eq:app-pricing}
\end{equation}
the separation problem of $D_{\mathcal R}$: a route with $rc_r(v)<0$ is a violated dual constraint. Column generation iterates: solve
$\mathrm{RMP}(T)$, solve \eqref{eq:app-pricing} at $v_T$, stop if $m(v_T)\ge 0$, otherwise add a
batch of routes with negative reduced cost to $T$ \citep{barnhart1998branch,
lubbecke2005selected}.

\begin{proposition}[Optimality]
\label{prop:app-opt}
\textup{(i)} If $m(v_T)\ge 0$, then $\lambda_T$ extended by zeros is optimal for
\eqref{eq:app-cvrp-master} and $z_T=z_{\mathrm{DW}}$. \textup{(ii)} If $z_T=z_{\mathrm{DW}}$,
then $F_T\cap D_{\mathcal R}\neq\emptyset$; the vertex $v_T$ returned by the simplex method need
not lie in $D_{\mathcal R}$.
\end{proposition}
\begin{proof}
(i) $v_T$ is feasible for the dual of \eqref{eq:app-cvrp-master} with objective $z_T$, the value
of the feasible primal solution $\lambda_T$, so both are optimal by weak duality. (ii) An optimal
dual $v^{*}$ of the full master is feasible for the dual of $\mathrm{RMP}(T)$ with objective
$z_{\mathrm{DW}}=z_T$, hence $v^{*}\in F_T\cap D_{\mathcal R}$; $F_T$ may nevertheless have
vertices outside $D_{\mathcal R}$, which is the situation discussed after \eqref{eq:dualpoly}.
\end{proof}

\begin{proposition}[Lagrangian bound]
\label{prop:app-lagr}
Let $\kappa$ bound $\sum_{r}\lambda_r$ over the feasible solutions of \eqref{eq:app-cvrp-master}.
For every $u\in\mathbb R^{n}$ and $\sigma\ge 0$,
\begin{equation}
z_{\mathrm{DW}}\ \ge\ L(v)\ =\ \sum_{i\in C}u_i+K_{\min}\sigma+\kappa\,\min\{0,\,m(v)\}.
\label{eq:app-lagr}
\end{equation}
\end{proposition}
\begin{proof}
For a feasible $\lambda$ write $s=\sum_r\lambda_r$, so that $K_{\min}\le s\le\kappa$. Since
$\sum_r a_{ir}\lambda_r=1$ for every $i$ and $rc_r(v)\ge m(v)$,
\begin{align*}
\sum_r c_r\lambda_r
&=\sum_i u_i\sum_r a_{ir}\lambda_r+\sigma\sum_r\lambda_r+\sum_r rc_r(v)\lambda_r
 \;=\;\sum_i u_i+\sigma s+\sum_r rc_r(v)\lambda_r\\
&\ge\sum_i u_i+K_{\min}\sigma+\min\{0,m(v)\}\,s
 \;\ge\;\sum_i u_i+K_{\min}\sigma+\kappa\,\min\{0,m(v)\}=L(v),
\end{align*}
using $\sigma\ge 0$ in the first inequality and $\min\{0,m(v)\}\le 0$ in the second.
\end{proof}
Every route covers at least one customer and every customer is covered once, so $\kappa=n$ and
\eqref{eq:app-lagr} is the bound $L$ of \eqref{eq:lagr}. The bound is computed by the exact
pricing call that finds the columns: the running maximum of the certified bounds is nondecreasing,
$z_T$ is nonincreasing in $T$, and the two meet when $m(v_T)\ge 0$. Every dual point has a bound,
feasible or not, which is what allows a stabilization center to be selected by its bound.

\paragraph{Degeneracy and smoothing.}
The face $F_T$ is in general not a singleton, and successive $v_T$ can change substantially
while $z_T$ barely moves, so that the tail of column generation stretches
\citep{lubbecke2005selected, dumerle1999stabilized}. Wentges smoothing \citep{wentges1997weighted} prices at the query
$q_t=(1-\alpha_t)v_t+\alpha_t c_t$, with $c_t=(c_{t,C},c_{t,\mathrm{veh}})$ the center and
$\alpha_t\in[0,1)$ the weight, which extends \eqref{eq:smooth} to the vehicle coordinate, and
admits a returned route $r$ only if $rc_r(v_t)<-\epsilon$ at the raw dual. An exact smoothed query
that returns no route admissible at $v_t$ is a \emph{mis-price}; it triggers the next rung of the
ladder
\begin{equation}
\alpha_{(j)}=\max\{0,\ 1-(j+1)(1-\alpha_t)\},\qquad j=0,1,\dots,
\label{eq:app-ladder}
\end{equation}

\begin{table}[h]
\centering\footnotesize\setlength{\tabcolsep}{6pt}
\caption{Constants of the smoothing rule, RouteOpt's defaults, used unchanged in every configuration: the initial weight, the weight step and cap of \eqref{eq:alpha}, the pricing tolerance of the admission test, and the tolerances of \eqref{eq:update} and \eqref{eq:alpha}.}
\label{tab:app-smooth-constants}
\begin{tabular}{lcccccc}
\toprule
constant & $\alpha_0$ & $\eta$ & $\bar\alpha$ & $\epsilon$ & $\epsilon_L$ & $\epsilon_g$ \\
\midrule
value & $0.5$ & $0.1$ & $0.9$ & $10^{-5}$ & $10^{-6}$ & $10^{-9}$ \\
\bottomrule
\end{tabular}
\end{table}

and termination requires a complete exact call at $\alpha_{(j)}=0$ that returns no route with
$rc_r(v_t)<-\epsilon$, which certifies $m(v_t)\ge-\epsilon$ \citep{pessoa2018automation}. At the
end of each exact-pricing sequence, the best complete query determines the center update of
\eqref{eq:update}, the center being replaced only when its certified bound improves by more than
$\epsilon_L$, and the last complete query determines the weight update of \eqref{eq:alpha}. Because admission uses the raw dual, smoothing changes the sequence $T$ and the
time, never $z_{\mathrm{DW}}$.

\paragraph{Heuristic and exact pricing.}
Pricing is solved by dynamic programming over labels, and labels are discarded under a dominance
relation $\preceq$ (Appendix~\ref{app:bpc-cvrp}). The exact level uses a relation
$\preceq_{\mathrm E}$ under which every completion of a discarded label is matched by a completion
of its dominator with no larger reduced cost, so that it returns a minimizer of
\eqref{eq:app-pricing}; the heuristic levels use coarser relations
$\preceq_{\mathrm E}\subseteq\preceq_{\mathrm H}\subseteq\preceq_{\mathrm L}$ that compare fewer
label components, discard more labels and may therefore miss the minimizer. A heuristic call returns
a subset of the routes with $rc_r(v)<0$ and can never certify $m(v)\ge 0$; termination requires an
exact call. \emph{Root pricing}, the quantity measured in this paper, is the first column generation
from the initial columns to the exact certificate, before any cut is separated.

\paragraph{Cuts and branching.}
After the initial cut-free root column generation, root cut rounds strengthen the bound with valid
inequalities and branching enforces integrality, both imposed inside the pricing problem. Cuts on the edge flow
$x_e=\sum_r b_{er}\lambda_r$, such as rounded capacity cuts, are \emph{robust}: their multipliers
modify the edge costs and leave the structure of pricing unchanged \citep{fukasawa2006robust}. Cuts
on the columns, such as subset-row and limited-memory rank-1 cuts, are \emph{non-robust}: each adds
a state component to the labels and modifies the dominance test \citep{jepsen2008subset,
pecin2017improved}. Edge branching is enforced by deleting forbidden arcs or by adding master rows whose dual
multipliers modify the pricing costs; reduced-cost arc
elimination \citep{irnich2010path} and route enumeration \citep{baldacci2008exact} complete the
toolbox surveyed by \citet{costa2019exact} and assembled in generic form by
\citet{pessoa2020generic}. Subsequent cut rounds and branching nodes reuse the columns generated by the initial root column
generation, which is the quantity measured in this paper.

\subsection{Two typical tasks: routing and scheduling}
\label{app:bpc-tasks}

In both families a column is the plan of one resource, a vehicle's route or a machine's schedule,
and the master covers a set of demands, customers or jobs. The pricing problems differ in kind:
routing prices by a resource-constrained shortest path over a graph, relaxed from elementarity by
ng-routes and solved by bucket-graph labeling with a dominance relation
\citep{baldacci2011new, sadykov2021bucket, pessoa2020generic}; the scheduling formulation used here
prices by a subset-selection dynamic program over jobs whose state is the accumulated processing
time \citep{vandenakker1999parallel, yu2026upmsbpc}. The learned components of this paper touch neither pricing problem; they generate column pools
and initialize stabilization centers. The two cases below fix what a column, a dual and a pricing call are in each family.

\subsection{Case 1: capacitated vehicle routing in RouteOpt}
\label{app:bpc-cvrp}

\paragraph{Instance and routes.}
Let $V=C\cup\{0\}$ with $|C|=n$, symmetric distances $d_{ij}$, demands $q_i$ and capacity $Q$. A
route $r=(0,i_1,\dots,i_k,0)$ visits customers $i_1,\dots,i_k$, has load $q(r)=\sum_h q_{i_h}\le Q$
and cost $c_r=\sum_{(i,j)\in r}d_{ij}$. A vehicle-indexed formulation separates the route-feasibility constraints by vehicle and has the
block structure of \eqref{eq:app-compact}; the master \eqref{eq:app-cvrp-master} uses anonymous
ng-route columns, defined next, and the valid vehicle-count inequality \citep{fukasawa2006robust,
pecin2017improved}.

\paragraph{ng-routes.}
Each customer $i$ carries a neighborhood $N_i\subseteq C$ with $i\in N_i$ and $|N_i|=\Delta$
($\Delta=8$ in the deployed configuration). Along a route the
\emph{ng memory} is defined by
\begin{equation}
\Pi_1=\{i_1\},\qquad \Pi_{h+1}=\big(\Pi_h\cap N_{i_{h+1}}\big)\cup\{i_{h+1}\},
\label{eq:app-ngmem}
\end{equation}
and $r$ is an \emph{ng-route} if $i_{h+1}\notin\Pi_h$ for every $h$: a customer may be revisited
only after the route has passed through a customer whose neighborhood does not contain it
\citep{baldacci2011new}. Every elementary route is an ng-route, and the ng-routes coincide with
the elementary routes when $N_i=C$ for all $i$, so enlarging the neighborhoods strengthens the
relaxation; heuristic columns from a metaheuristic are elementary and hence valid columns of
\eqref{eq:app-cvrp-master}.

\paragraph{Labeling.}
Put $u_0=0$ and $\bar d_{ij}=d_{ij}-u_j$, so that $rc_r(v)=\sum_{(i,j)\in r}\bar d_{ij}-\sigma$. A
\emph{label} is a tuple $L=(i,\,q,\,\Pi,\,\bar c)$: the last customer $i$ of a partial route from
the depot, its load $q$, its ng memory $\Pi$ and its accumulated cost $\bar c=\sum\bar d$ along the
partial route. The initial label is $(0,0,\emptyset,0)$; the extension of $L$ along arc $(i,j)$ is
feasible if $j\notin\Pi$ and $q+q_j\le Q$, and produces
\begin{equation}
L'=\big(j,\ q+q_j,\ (\Pi\cap N_j)\cup\{j\},\ \bar c+\bar d_{ij}\big);
\label{eq:app-extend}
\end{equation}
a label at $i$ closes to the route of reduced cost $\bar c+d_{i0}-\sigma$, and $m(v)$ is the
minimum over closed labels. Under symmetric distances RouteOpt forms routes by joining a forward partial route with the
reversal of another forward partial route over an edge $(i,j)$: with the label definitions above,
the join of $L_1$ at $i$ and $L_2$ at $j$ is feasible if $q_1+q_2\le Q$ and the concatenated route
satisfies the ng condition, and has reduced cost $\bar c_1+\bar c_2+d_{ij}-\sigma$.

\paragraph{Dominance.}
For two labels at the same customer, $L_1\preceq_{\mathrm E}L_2$ if
\begin{equation}
\bar c_1\le\bar c_2,\qquad q_1\le q_2,\qquad \Pi_1\subseteq\Pi_2 .
\label{eq:app-dom}
\end{equation}
\begin{proposition}[Dominance]
\label{prop:app-dom}
If $L_1\preceq_{\mathrm E}L_2$, then for every feasible completion of $L_2$ the same completion is
feasible for $L_1$ and yields a route with no larger reduced cost; hence $L_2$ can be discarded
without changing $m(v)$.
\end{proposition}
\begin{proof}
Feasibility of an extension requires $j\notin\Pi$ and $q+q_j\le Q$, both monotone in
$(q,\Pi)$; the memory update \eqref{eq:app-ngmem} preserves $\Pi_1\subseteq\Pi_2$ and the load
update preserves $q_1\le q_2$, so the conditions hold along the whole completion, and the cost
difference $\bar c_1-\bar c_2\le 0$ is carried unchanged. The same argument applies to the join.
\end{proof}
In the cut-free root comparisons, exact pricing uses \eqref{eq:app-dom}. With non-robust cuts,
dominance also accounts for their states and dual contributions; the heuristic levels use the
coarser relations described in Appendix~\ref{app:bpc-cg}.

\paragraph{Bucket graph.}
Fix a load step $\Delta_q$ and let bucket $B(i,k)$ hold the labels at customer $i$ with load in
$[k\Delta_q,(k+1)\Delta_q)$. Buckets are processed in increasing $k$; a label in $B(i,k)$ can only
be dominated by labels in $B(i,k')$ with $k'\le k$, so the dominance check for a new label is
restricted to the current bucket and, through a lower bound on the reduced cost of the earlier
buckets of the same customer, to a cross-bucket test; the extension \eqref{eq:app-extend} moves a
label along a \emph{bucket arc} from $(i,k)$ to $(j,k')$ with $k'$ the bucket of $q+q_j$, and \emph{jump arcs} advance the resource to a later bucket of the same vertex before traversing a
retained outgoing arc \citep{sadykov2021bucket}. In RouteOpt's own implementation each
arrival is checked against the bucket as it stands and inserted, so that the arrivals to a bucket
form a chain; Appendix~\ref{app:gpu} is about removing this dependence.

\paragraph{Smoothing and the root.}
The root loop studied here runs the Wentges rule of Appendix~\ref{app:bpc-cg} with the center updates, the weight adaptation and the ladder \eqref{eq:app-ladder} of Section~\ref{sec:m-centre}. The paper's measurements stop at the first
exact certificate of the root; after it, RouteOpt continues as a branch-price-and-cut solver
\citep{routeopt}: rounded capacity cuts are separated heuristically with the CVRPSEP routines, limited-memory rank-1 cuts involving up to five customer rows by seed-set enumeration and local
search \citep{pecin2017limited}, branching is on edges with three-phase strong branching whose candidates are screened by a
learned model \citep{you2026two}, and reduced-cost arc elimination and route enumeration are
applied once the gap permits. Root pricing is the first cut-free column generation up to the exact
certificate, with no cut, no branching decision and no arc elimination. When the root loop
separates rounded capacity cuts, the learned center is reinstalled at the start of every round,
while LIGHT-level smoothing activates only after a fixed number of iterations within the round; the
solver comparisons of Section~\ref{sec:experiments} and Appendix~\ref{app:results} are cut-free,
so this rule is stated for completeness, and the CPU profile of Appendix~\ref{app:gpu-bottleneck}
is the one measurement taken on a cut-loaded root.

\subsection{Case 2: unrelated parallel machine scheduling}
\label{app:bpc-upms}
\label{app:upms:setting}

\paragraph{Instance, columns and master.}
Jobs $J=\{1,\dots,n\}$ are assigned to machines $M=\{1,\dots,m\}$; job $j$ takes time $p_{kj}$ on
machine $k$ and carries a weight $w_j$, and the objective is $\sum_j w_jC_j$ with $C_j$ the
completion time of $j$. A column is a \emph{single-machine schedule} $(k,S)$, $S\subseteq J$,
sequenced in the weighted-shortest-processing-time order of machine $k$
($p_{kj}/w_j$ nondecreasing), which is optimal within a fixed job set; its cost is
$c_k(S)=\sum_{j\in S}w_j\,C_j(k,S)$ with $C_j(k,S)=\sum_{l\in S,\ l\preceq_k j}p_{kl}$. Schedule
columns originate in the identical-machine setting of \citet{vandenakker1999parallel}; the machine-indexed master of \citet{yu2026upmsbpc}, on which the experiments of
Section~\ref{sec:exp-upms} build with the deviations described below, is
\begin{equation}
\min_{\lambda\ge 0}\Big\{\sum_{k\in M}\sum_{S\subseteq J} c_k(S)\,\lambda_{k,S}:\
\sum_{k\in M}\sum_{S\ni j}\lambda_{k,S}\ \ge\ 1\ (j\in J),\ \
\sum_{S\subseteq J}\lambda_{k,S}\ \le\ 1\ (k\in M)\Big\},
\label{eq:app-upms-master}
\end{equation}
with duals $\pi_j\ge 0$ on the jobs and $\sigma_k\le 0$ on the machines and reduced cost
$rc_{k,S}=c_k(S)-\sum_{j\in S}\pi_j-\sigma_k$; the formulation of \citet{hijazi2026improving}
below imposes equality on the job rows, so that its job duals are unrestricted in sign. With singleton schedules as the only initial columns and at
most one schedule per machine, the initial restricted master needs artificial covering variables
when $n>m$.

\paragraph{Pricing by dynamic programming.}
For machine $k$ index the jobs in its weighted-shortest-processing-time order and let
$F_k(j,t)$ be the minimum of $\sum_{l\in S}(w_lC_l-\pi_l)$ over subsets $S$ of the first $j$ jobs
with total processing time $t$; then
\begin{equation}
F_k(j,t)=\min\big\{F_k(j-1,t),\ \ F_k(j-1,t-p_{kj})+w_j\,t-\pi_j\big\},
\label{eq:app-upms-dp}
\end{equation}
with $F_k(0,0)=0$ and $+\infty$ assigned to every infeasible state, including all states with
$t<0$, because appending $j$ to a schedule of total time $t-p_{kj}$ completes it at time $t$. The
minimum reduced cost is $rc^{\min}(\pi,\sigma)=\min_{k}\big[\min_t F_k(n,t)-\sigma_k\big]$,
computed exactly in
$O(n\sum_j p_{kj})$ per machine for integer processing times: a pseudo-polynomial table with no
dominance rule. In the implementation used here the recursion is vectorized. The reference implementation of
\citet{yu2026upmsbpc} shares the master \eqref{eq:app-upms-master} and uses Wentges smoothing with
$\alpha_0=0.5$ and Lagrangian-bound center updates; its mis-pricing update differs from
\eqref{eq:app-ladder}, and it disables smoothing once the weight reaches zero, whereas the harness
of this paper restarts its retry sequence at each iteration.

\paragraph{The published learned column-generation setting.}
The comparison of Section~\ref{sec:exp-upms} runs inside the released code of
\citet{hijazi2026improving}, who replace the pricing oracle by a pointer transformer and keep an
exact dynamic program of the form \eqref{eq:app-upms-dp} as the fallback that preserves the
optimality guarantee. Their setting differs from \eqref{eq:app-upms-master} in three respects that
matter for reading the results: the master is a set-partitioning master without artificial
variables, each job covered exactly once and each machine used at most once; the restricted master
is seeded with one hundred random job subsets per machine; and no dual stabilization is used.
Their contribution is on the pricing side; Section~\ref{sec:exp-upms} combines their learned
pricer with column initialization and dual stabilization inside one implementation.

\paragraph{The learned center for scheduling.}
The center of Section~\ref{sec:exp-upms} is the scheduling analogue of the model of
Appendix~\ref{app:learn-centre-train}: a bipartite set-attention network over jobs and machines,
with cross-attention biased by the processing times, that reads the instance data alone and
predicts the certified root duals in the scale-free units $\pi_j/(w_j\bar L)$ and $\sigma_k/C_0$,
where $\bar L$ is the mean machine load and $C_0=\bar L\sum_j w_j$; it was trained on $168$
instances of the benchmark generator of \citet{yu2026upmsbpc}, selected on a validation split,
and not retrained on the distribution of \citet{hijazi2026improving}. The prediction is projected
onto $\pi\ge 0$, $\sigma\le 0$ and installed at iteration $0$ together with its own Lagrangian
value from one exact sweep, after which the Wentges rule runs unchanged.


==> sections/app_gpu.tex <==
\section{GPU exact pricing in detail}
\label{app:gpu}

\subsection{Bucket-graph labeling and the dominance test}
\label{app:gpu-bucket}

RouteOpt prices by bucket-graph labeling \citep{sadykov2021bucket}. A label is a partial route
leaving the depot together with its reduced cost, its resource consumption, its ng memory and, in
the tree, its cut states. The labels at a customer are kept in buckets indexed by a resource
interval, and the algorithm processes buckets in resource order, extending each label along the
bucket arcs and the jump arcs into the buckets of its successors. In RouteOpt's own implementation this
is a \emph{push}: an extended label arrives at its target bucket and is checked there against the
bucket's move-to-front list of stored labels, with early exit once a dominator is found; before a
stored label is extended, a cross-bucket check compares it with the earlier buckets of the same
customer through reduced-cost prefix bounds; buckets are sorted by reduced cost when their level is
done. The predicate compares resources, tests ng-set inclusion and, with cuts, checks a
reduced-cost gap corrected by the cut duals; the LIGHT and HEAVY levels use weaker predicates,
which is why they keep few labels and run quickly. Because every arrival is checked against the
bucket as it stands at that moment and changes it, the arrivals to a bucket form a chain; this is
the sequential dependence the backend removes. Under symmetry RouteOpt labels forward to the meet
point and joins two forward half-routes.

\subsection{Where the time goes}
\label{app:gpu-bottleneck}

Table~\ref{tab:app-gpuprofile} is the CPU profile that motivated the backend design of
Section~\ref{sec:m-gpu}, measured on vanilla RouteOpt at the root of Vrp-Set-X instances: the four
dominance components together account for close to half of the profiled root-execution self
cycles, of which \gpuProfDomCut{} points are cut-state dominance and absent from the cut-free root
measured in this paper, label extension for a small part, and one EXACT call evaluates orders of magnitude more
dominance predicates than a LIGHT or a HEAVY call while taking two orders of magnitude longer. On
the vanilla solver this concentration converts into little end to end, because exact pricing is a
minor share of the cut-free root there; prefill and the learned center change that share, as Section~\ref{sec:exp-gpu} and Figure~\ref{fig:provenance} show, and the exact level becomes the
stage where a further lever pays.

\begin{table}[!htb]
\centering\small
\caption{Where root labeling spends its time on the CPU: vanilla RouteOpt, single thread, cut-loaded root. Left: median self-cycle shares of profiled root execution over $35$ long-route runs; the dominance total sums the four components. Right: per-level counters on the root of X-n228-k23.}
\label{tab:app-gpuprofile}
\begin{tabular}{@{}lr@{\hskip 14pt}lrrr@{}}
\toprule
kernel & self \% & level & calls & s / call & predicates / call \\
\midrule
in-bucket dominance loop            & \gpuProfDomInBucket{} & LIGHT & \gpuLevelCallsLight{} & \gpuLevelSecPerCallLight{} & \gpuLevelPredLight{} \\
dominance core (load, ng subset)    & \gpuProfDomCore{} & HEAVY & \gpuLevelCallsHeavy{} & \gpuLevelSecPerCallHeavy{} & \gpuLevelPredHeavy{} \\
cut-state dominance                 & \gpuProfDomCut{} & EXACT & \gpuLevelCallsExact{} & \gpuLevelSecPerCallExact{} & \gpuLevelPredExact{} \\
cross-bucket dominance              & \gpuProfDomCross{} &       &     &      & \\
\emph{dominance, total}             & \emph{\gpuProfDomTotal{}} & & & & \\
label extension                     & \gpuProfExtend{} & & & & \\
cut-state update                    & \gpuProfCutUpdate{} & & & & \\
concatenation                       & \gpuProfConcat{} & & & & \\
LP solver                           & \gpuProfLP{} & & & & \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Removing the sequential dependence}
\label{app:gpu-backend}

The backend keeps the contract of the CPU pricer and changes the shape of the computation. At
each resource level it expands the current frontier and groups the candidates by target bucket;
same-level candidates form the next wave of that level, and candidates for later levels wait for
theirs. The candidates of one bucket in a wave form a segment, tested in three stages. Stored
labels against candidates: each candidate independently, stopping at its first dominator, whose
stored label is marked as a witness. Candidates against candidates in the canonical order
(reduced cost, resources, ng cardinality, generation index): the serial reference accepts
candidates in that order, and the exact GPU mode compares each candidate in parallel against all
earlier candidates that survived the first stage. Surviving candidates against the stored labels,
with marked witnesses exempt from deletion. A repair pass then restores any deleted candidate
without a surviving direct dominator. Every deleted label therefore has a dominator alive at the
end of the wave, an invariant maintained by retaining the stored labels that serve as deletion
witnesses and stronger than what RouteOpt's own implementation offers under tolerance. Label state is
held in structure-of-arrays form; shared-memory tiles reuse candidate prefixes across the
comparisons of a block; an optional warp-per-segment path for small segments exists and is
disabled in the deployed configuration; the cross-bucket filter runs one warp per frontier label
and uses the same reduced-cost prefix bound as the CPU. Label extension, dominance testing and the
forward--forward join run on the GPU; route reconstruction, deduplication by canonical route
identity and the final selection of returned columns run on the CPU, and with stable numbering,
canonical sorting and fixed scan rules the output does not depend on scheduling. The heuristic
levels, the master and the cut loop stay on the CPU, and dispatch sits inside the exact level, so
the column-generation loop is unchanged.

\subsection{Certification and safeguards}
\label{app:gpu-safeguards}

The backend runs only where its preconditions hold, namely symmetric instances and an ng bit-set
width within the compiled bound, with automatic CPU fallback otherwise. Every returned column is
re-priced on the CPU at the query $q_t$ actually used, since the solver prices at $q_t$ and
admits at $u_t$, and mismatches are counted rather than silently accepted. An empty backend
answer is not accepted as a certificate: before column generation terminates, one CPU EXACT call
re-proves the same dual, so the root bound of a GPU run is certified by the CPU pricer. The
backend's output policy is aligned with the CPU truncation rule, since a different rule changes
how many columns a call returns and hence how many calls the loop makes. Correctness is checked by
comparing final root bounds across arms and, in a diagnostic configuration, the returned column
sets call by call, and the completed arms of every comparison in this paper must report the same
root bound.

\subsection{What the backend buys per call}
\label{app:gpu-percall}

Table~\ref{tab:app-gpucall} reconciles the same EXACT calls on the CPU and on the GPU: each call is served
by the backend and, in the same process on the same input, by RouteOpt's own labeling, so machine
and contention cancel. Table~\ref{tab:app-gpucall-devices} extends the comparison to three cards
on the learned stack, for the \gpuHwN{} Vrp-Set-X instances with the longest exact pricing time in a preliminary sweep, two
of which lie below the $300$-customer floor of the main panel: per instance, the median per-call seconds of steady-state exact calls on the
single CPU thread and on each card, with the first call, which includes GPU initialization, and
the last call, which is the CPU re-proof by design, excluded. Bounds agree on
\gpuHwBoundsSame{} instances and the three cards' exact-call counts on \gpuHwCallsSame{}; only the exact-pricing clock is compared, which leaves out the LP solves, run on the CPU on every card. Section~\ref{sec:exp-gpu} quotes the medians over instances of these ratios.

\begin{table}[!htb]
\centering\small
\caption{The same EXACT calls served by RouteOpt's labeling on the CPU and by the backend on an L4, first cut-free CG of five Vrp-Set-X instances. The last column estimates the end-to-end gain by subtracting the measured pricing time, a speed-up factor with higher better; it is not a separate vanilla run.}
\label{tab:app-gpucall}
\begin{tabular}{@{}lrrrrr@{}}
\toprule
instance & EXACT calls & CPU (s) & L4 (s) & CPU / L4 & end-to-end (est.) \\
\midrule
\gpuTableCallRows
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!htb]
\centering\footnotesize
\caption{Per-instance exact pricing on three GPUs, learned stack, the \gpuHwN{} X instances with the longest exact pricing time: steady-state exact calls, median seconds per call on one CPU thread and on each card, and their ratios. Bounds agree on \gpuHwBoundsSame{} instances and call counts on \gpuHwCallsSame{}.}
\label{tab:app-gpucall-devices}
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lrrrrrrrr}
\toprule
instance & calls & CPU (s) & L4 (s) & B200 (s) & RTX (s) & B200/L4 & RTX/L4 & L4/CPU \\
\midrule
\gpuHwTableCallRows
\bottomrule
\end{tabular}
\end{table}


==> sections/app_learning.tex <==
\section{The learning components in detail}
\label{app:learning}
\label{app:method}

Both learned components read the instance file and nothing else, run once before column
generation starts, and hand the solver an object it already uses: a pool of routes for the lazy
archive of Section~\ref{sec:m-prefill}, and an initial center for the smoothing rule of
Section~\ref{sec:m-centre}. This appendix describes each component as a training problem, with its
architecture, features, labels and training parameters, and as an inference step, with what the
prediction becomes inside the solver. The shared label set and its splits are in
Appendix~\ref{app:learn-data}.

\subsection{Learning to prefill}
\label{app:learn-prefill}

\subsubsection{Training}
\label{app:learn-prefill-train}

\paragraph{Model architecture.}
The deployed scorer $f_\theta$ of \eqref{eq:heat} is a message-passing network over the candidate
graph $E(I)$, the $20$ nearest neighbors of each customer plus the depot edges. Node inputs are the
position relative to the depot in units of the mean depot distance, the demand fraction $q_i/Q$,
the depot distance in the same units, the candidate degree divided by $20$, and a depot flag; edge
inputs are the $26$ instance-only edge features below. Three rounds of messages are built from
$h_i+h_j$, $h_i\odot h_j$ and $e_{ij}$, hence symmetric in the endpoints, at width $192$, followed
by an edge head. The graph is constructed from the instance alone and is therefore identical during
training and at generation time. Table~\ref{tab:app-edge-scorer} lists the architecture and the
training parameters.

\paragraph{Features.}
The $26$ edge features are instance-only quantities: normalized edge and depot distances,
nearest-neighbor ranks and membership indicators of the two endpoints, the depot-centered angular
separation of the endpoints, the normalized savings term $d_{0i}+d_{0j}-d_{ij}$, the endpoint
demands, a depot-edge flag and instance context. No feature depends on a solution, a dual or a
pool, so the same feature extractor serves training and deployment.

\paragraph{Labels.}
The label of an edge is its \emph{heat} $\nu_e$ of \eqref{eq:heat}: among the routes of the
instance's reference pool that price out at the reference center, the fraction of those visiting
$i$ or $j$ that traverse $e$. The reference pool is the metaheuristic pool of the instance, built by hybrid genetic search with
three seeds and a time and route-count budget that grows with the instance size, and the reference
center is the tree-predicted center \textsc{Cg} of the instance, the deployed center at the time the
labels were computed, so that the heated edges are the edges used by the routes that a plausible
iteration-$0$ center asks for; a route prices out when its reduced cost at that center is below $-10^{-9}$. The
supervised edge set $H(I)$ adds the reference-pool edges to $E(I)$, so that the supervised set
includes reference-pool edges outside the message-passing graph while message passing uses only the
instance-derived candidate graph, and the regression target is $\sqrt{\nu_e}$, which spreads the
mass of the many lightly heated edges. Training uses the training split of
Appendix~\ref{app:learn-data} and excludes instances with fewer than $50$ negative-reduced-cost
reference routes, leaving $192$ of the $200$ training instances.

\paragraph{Training parameters.}
Table~\ref{tab:app-edge-scorer} gives the optimizer, schedule and selection rule. The checkpoint
is the epoch with the best validation Spearman rank correlation with $\nu$. Offline rank
correlation is the selection statistic and nothing more; the pool is evaluated end to end in
Appendix~\ref{app:results-pool}.

\begin{table}[!htb]
\centering\small
\caption{Deployed edge scorer: architecture and training parameters.}
\label{tab:app-edge-scorer}
\begin{tabular}{p{0.28\textwidth}p{0.64\textwidth}}
\toprule
item & value \\
\midrule
graph & $20$-NN candidate graph plus depot edges, built from the instance file; identical at
training and at generation time \\
node inputs & relative position and depot distance in units of the mean depot distance, $q_i/Q$,
candidate degree$/20$, depot flag \\
edge inputs & the $26$ instance-only edge features \\
message passing & three rounds at width $192$; messages from $h_i+h_j$, $h_i\odot h_j$, $e_{ij}$;
edge head; no dropout \\
parameters & $1\,432\,321$ \\
target and loss & $\sqrt{\nu_e}$ on $H(I)$, squared error \\
training set & $192$ of the $200$ training instances (instances with fewer than $50$
negative-reduced-cost reference routes excluded) \\
optimizer & AdamW, learning rate $8\times10^{-4}$, weight decay $0$, cosine annealing to
$0.01\times$ the initial rate, batches of $16$ instances, gradient-norm clip $5$, seed $0$ \\
epochs and selection & $260$ epochs, no early stopping; checkpoint with the best validation
Spearman rank correlation (epoch $158$) \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Inference: from the heat map to the archive}
\label{app:learn-prefill-infer}

\paragraph{The generator.}
Algorithm~\ref{alg:gen} turns the heat map into a pool of routes with the constants of
Table~\ref{tab:app-constructor}. The deployed pools are built under a time budget of ten seconds per instance, four independent seeds running in parallel and merged at the end by customer set. Routes are deduplicated by customer set, keeping the cheapest
ordering seen, so the pool holds distinct columns by construction; a costlier ordering of the same
customer set is a dominated column.

\begin{table}[!htb]
\centering\small
\caption{Learned constructor: constants of Algorithm~\ref{alg:gen} in the deployed configuration.}
\label{tab:app-constructor}
\begin{tabular}{p{0.28\textwidth}p{0.64\textwidth}}
\toprule
item & value \\
\midrule
time budget $T$ & ten seconds per instance, shared by the seeds \\
seeds & $W=4$ independent seeds in parallel, merged by customer set; random seed $42$ \\
neighborhood $\mathcal N(i)$ & edges of the $20$-NN graph among the $12$ highest-scoring candidates
at either endpoint \\
floors and exponents & $\delta=10^{-9}$ on the depot heat, $\delta'=10^{-12}$ on the walk weights,
coverage exponent $\gamma=2$ \\
tour sampling & $\tau$ uniform on $\{2,4,8,16\}$ per tour; multiplicative noise $e^{0.15Z}$,
$Z\sim\mathcal N(0,1)$, per step; nearest-unvisited fallback may leave $E(I)$ \\
tour to routes & neighbor-list 2-opt on the giant tour; optimal split \citep{prins2004simple} under
capacity and a route-length bound of $\max\{25,\lceil 3n/K_{\min}\rceil\}$ customers; intra-route
2-opt (Polish); split-and-search twice per tour \\
local search & relocate, swap and 2-opt* in up to three passes per route set \\
stopping rule & a seed stops when $400$ consecutive tours add no new customer set \\
deduplication & by customer set, cheapest ordering kept \\
archive batch & at most $B=300$ routes offered per pricing round, each route once \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{How the pool is used.}
The pool never enters the initial restricted master; it is a lazy archive that supplies columns
at pricing time by \eqref{eq:archive}. At every pricing round, before any labeling, the archive
offers at most $B=300$ routes, the most negative at the smoothed query $q_t$ among those not yet
offered, and the solver admits those with $rc_r(u_t)<-\epsilon$ at the raw dual, the same test a
generated column must pass; each route is offered once, and the labeling call of that round is
skipped when at least one route is admitted. On instrumented development instances the
archive served \archiveFastPathLo{} to \archiveFastPathHi{}\,\% of LIGHT rounds this way; when it
supplies no admissible column, the solver resumes labeling. Because admission uses the solver's
own test, the archive changes the trajectory of column generation and not the value it converges
to, and because the routes are never in the initial master, no basis is imposed on the first
simplex solve; Appendix~\ref{app:results-earlier} records why preloading the same kind of columns
into the initial master fails.

\paragraph{Cost.}
In a dedicated timing study on an uncontended node, excluding coverage instrumentation that a
deployment does not run, the learned generator's whole-command wall is \poolWallCleanNLo{} to
\poolWallCleanNHi{} of the metaheuristic pool's; Appendix~\ref{app:results-pool} compares the learned pool with a heuristic
pool whose generation time is included.

\subsection{Learning the dual center}
\label{app:learn-centre}

\subsubsection{Training}
\label{app:learn-centre-train}

\paragraph{Model architecture.}
The deployed center \textsc{Cn} is a set transformer $g_\varphi$ over customer tokens plus an
instance-context token: three pre-layer-norm blocks of multi-head attention at $d=128$ with eight
heads and dropout $0.1$, a geometric additive bias on the attention logits that encodes the
distance between the two customers, a per-customer softplus head for the direction and a scalar
head for the log magnitude of \eqref{eq:centreloss}. The vehicle row of the center comes from a
gradient-boosted tree model on instance context, and the tree center \textsc{Cg}, gradient-boosted
trees that predict each customer independently from the same features, is the tree-based
alternative to the direction model. Table~\ref{tab:app-centre-model}
lists the architectures and the training parameters.

\paragraph{Features.}
The $53$ per-customer features are the depot distance in raw, normalized and rank form, the demand
and the demand fraction $q_i/Q$, the distance to the customer centroid, neighborhood statistics at
two neighborhood sizes, and instance context such as $n$, $K_{\min}$, $Q$, $n/K_{\min}$ and the
dispersion of depot distances and demands. Features derived from the root LP value are excluded,
so that the model needs no solve, and the generator-family digits of the label instances are
dropped so that the model applies outside that generator. The trees use the same features; the
vehicle-row model uses nine instance-context features.

\paragraph{Labels.}
The label of an instance is its certified optimal root dual $\pi^{*}$, customer block and vehicle
row, obtained as described in Appendix~\ref{app:learn-data}. The direction target is the
singleton-normalized coordinate $y_i=\pi^{*}_i/(2d_{0i})$, so that the network predicts each
customer's dual relative to the cost of serving it alone, and the magnitude target is the ratio
$\rho^{*}$ of the customer-dual norm to the singleton-cost norm of \eqref{eq:centreloss}; the
vehicle-row model regresses $\pi^{*}_{\mathrm{veh}}/\operatorname{mean}_i d_{0i}$ on the instance
context. Including the vehicle row, the median relative $L_2$ error of the predicted center on the
test split is \centreRelLtwoFull{}, against \centreRelLtwoTest{} for the customer block alone; the
paper's claim is not that this error is small but that the direction it encodes is a good initial
center, which Appendix~\ref{app:results-centre} tests against controls.

\paragraph{Training parameters and magnitude calibration.}
Table~\ref{tab:app-centre-model} gives the optimizer, schedule and selection rule; \textsc{Cn} was
selected on validation cosine after the box projection out of $87$ training runs of the same
family. A direction is installable only once it has a magnitude, and what the solver sees is the
magnitude after the box projection of \eqref{eq:install}, so the scale must be produced without
consulting the tree model at test time. The deployed calibration forms a target norm $T$ in log
space as the geometric mean of de-biased estimates available at test time, the scale heads of two
auxiliary networks of the same family and the norm predicted by a network trained under a plain
$L_2$ loss, and scales the direction by the factor for which the norm \emph{after} the box
projection equals $T$, found by bisection; when the target exceeds the norm of the box corner, the
corner itself is installed.

\begin{table}[!htb]
\centering\small
\caption{Deployed dual center: architectures and training parameters.}
\label{tab:app-centre-model}
\begin{tabular}{p{0.28\textwidth}p{0.64\textwidth}}
\toprule
item & value \\
\midrule
inputs & $53$ per-customer features plus an instance-context token, all computable from the
instance file \\
set transformer (\textsc{Cn}) & three pre-layer-norm blocks, $d=128$, eight heads, geometric additive
attention bias, dropout $0.1$; per-customer softplus direction head; scalar log-magnitude head;
$423\,834$ parameters \\
labels & $y_i=\pi^{*}_i/(2d_{0i})$ for the direction; $\rho^{*}=\|\pi^{*}_C\|_2/\|2d_0\|_2$ for
the magnitude \\
loss & \eqref{eq:centreloss} with $\beta=0.3$ \\
optimizer & AdamW, learning rate $10^{-3}$, weight decay $0.01$, batch $8$, ten warm-up epochs then
a cosine schedule, cap $220$ epochs, patience $29$, seed $0$; best epoch $44$ \\
selection & validation cosine after the box projection, out of $87$ runs of the same family \\
box projection & $0\le c_i\le\max(2d_{0i}-c_{\mathrm{veh}},0)$, with $c_{\mathrm{veh}}$ clipped at
$0$ \\
magnitude calibration & target norm $T$: geometric mean in log space of three de-biased estimates
(scale heads of two auxiliary set-transformer networks with $d=64$, four heads, two blocks; the norm
of a network of that architecture trained under a plain $L_2$ loss); $s$ by bisection so that
$\|\Pi_{\mathcal B}(sD_0\hat y)\|_2=T$; corner installed when $T$ exceeds the corner norm \\
vehicle-row model & histogram gradient-boosted trees, $200$ trees, depth $4$, learning rate $0.06$,
at least $5$ samples per leaf, seed $0$; target $\pi^{*}_{\mathrm{veh}}/\operatorname{mean}_i
d_{0i}$ on $9$ instance-context features \\
tree center (\textsc{Cg}) & histogram gradient-boosted trees, at most $400$ iterations with early
stopping on a $0.1$ validation fraction and patience $30$ ($369$ trees), depth $6$, learning rate
$0.06$, at least $40$ samples per leaf, $L_2$ regularization $1.0$, $255$ bins, seed $0$; same
$53$ features and labels \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Inference: from the prediction to the smoothing center}
\label{app:learn-centre-infer}

The predictor is evaluated once per instance, in process: feature construction takes a median of
\cfnNTennCFeatMed{}\,s and network inference \cfnNTennCCppMed{}\,s. The customer block is clipped to the singleton-based
box $\mathcal{B}$ of \eqref{eq:install} after scaling, the vehicle dual from the trees is clipped
at $0$, and the resulting $c_0$ is installed at the first pricing iteration. The solver certifies it by one exact pricing call at
$c_0$, whose outcome is the Lagrangian bound $L(c_0)$ of \eqref{eq:lagr}; the columns that call
prices out are dropped, so the center adds no column of its
own and acts only through the queries it shapes. This replaces the seeding exact call that the
stabilized baseline pays for its first center. From then on the rule of
Section~\ref{sec:bg-smoothing} runs unchanged: whenever a complete exact pricing improves the
Lagrangian bound, the center moves to that dual point by \eqref{eq:update}, and the weight adapts
by \eqref{eq:alpha}; the center is therefore \emph{not} held fixed after initialization. The
deployed configuration also carries the endgame switch, which sets $\alpha=0$ and stops
adaptation after two consecutive complete, non-retry exact calls that each admit between $1$ and
$99$ columns, and the LIGHT fallback: after an empty smoothed LIGHT query the solver retries at the
raw dual, and if that retry admits columns the remainder of the LIGHT phase prices at the raw
dual. Under cut separation the prediction would be reinstalled every cut round, a configuration
not used in this paper. The calibration above aims the center at a scale at which pricing stays
productive (Section~\ref{sec:m-centre}).

\subsection{Labels and data}
\label{app:learn-data}

The label set consists of $320$ instances of the XML generator \citep{queiroga2022xml}, $80$ each
at $100$, $200$, $300$ and $500$ customers, twenty per route-length class from medium to ultra
long, and none at $400$ customers, so that the XML400 instances of the evaluation panels are
unexposed to both learned components; no Vrp-Set-X instance is labeled. Each label instance was
solved at the root by vanilla RouteOpt, without prefilled columns, to the exact certificate, and the converged restricted master was written out with its basis. The label
$\pi^{*}$, customer block and vehicle row, is the basic optimal dual of that master, recovered by
re-solving the written program with primal simplex from the saved basis in zero iterations, and
accepted only if its objective matches the root value to a relative $10^{-7}$ and no reference-pool
route prices out at it beyond $10^{-6}$. A metaheuristic reference pool was built for every label instance and for every evaluation
instance with the same recipe. The
instances are split $200/60/60$ into training, validation and test instances, stratified into
sixteen groups by size and route-length class with split seed $20260913$; both learned components use the same instance split
and the same $60$ validation instances, the center training on all $200$ training instances and
selecting on validation cosine, the scorer retaining $192$ of them after the reference-route-count
filter and selecting on validation rank correlation. None of the \ablVfourMainInstN{} evaluation instances of Section~\ref{sec:experiments} is a training or validation instance of either model; its XML400 and Vrp-Set-X instances are not labeled at all.


==> sections/app_repro.tex <==
\section{Reproducibility}
\label{app:reproducibility}
\label{app:repro}

The routing experiments build on RouteOpt \citep{routeopt}, from whose released source the
vanilla solver and our fork are compiled with identical settings, and the scheduling case study
builds on the released code, instances and seeds of \citet{hijazi2026improving}. Linear programs
are solved with Gurobi $13.0.1$, and the GPU pricing backend is built with CUDA $12.9.1$. Every
source of randomness is seeded: the label set of Appendix~\ref{app:learn-data} is split with seed
$20260913$, and the pool generators, the smoothing rule, and the training runs use fixed seeds, those of the
generators and the training runs being listed in Appendix~\ref{app:learning}.


==> sections/app_results.tex <==
\section{Ablations and additional results}
\label{app:results}
\label{app:ablation}
\label{app:protocol}
\label{sec:exp-setup}
\label{app:classone}
\label{app:results-classone}
\label{app:results-ablation}
\label{app:results-failures}
\label{app:gpufail}
\label{app:results-upms}
\label{app:upms}
\label{app:upms:hijazi}
\label{app:upms:bench}
\label{app:headline83}
\label{sec:exp-headline}
\label{app:headline}
\label{app:results-earlier-panel}
\label{app:results-codesign}
\label{sec:learn-codesign}
\label{app:results-limits}
\label{sec:learn-summary}
\label{sec:related}
\label{sec:learning}
\label{app:results-ablations}

\input{sections/appendixD_ablations}

